Signed Graph Diffusion Network

Given a signed social graph, how can we learn appropriate node representations to infer the signs of missing edges? Signed social graphs have received considerable attention to model trust relationships. Learning node representations is crucial to effectively analyze graph data, and various techniques such as network embedding and graph convolutional network (GCN) have been proposed for learning signed graphs. However, traditional network embedding methods are not end-to-end for a specific task such as link sign prediction, and GCN-based methods suffer from a performance degradation problem when their depth increases. In this paper, we propose Signed Graph Diffusion Network (SGDNet), a novel graph neural network that achieves end-to-end node representation learning for link sign prediction in signed social graphs. We propose a random walk technique specially designed for signed graphs so that SGDNet effectively diffuses hidden node features. Through extensive experiments, we demonstrate that SGDNet outperforms state-of-the-art models in terms of link sign prediction accuracy.

==> 007impact.tex <==


Our work aims to learn high quality node representations for the link sign prediction task which predicts trust relationships between people who do not know each other. % well enough.
Our work contributes building healthy relationship between people which promotes mutual benefits and public interests in a social network.





%At the same time, this work may have some negative consequences because there is a risk of incorrectly predicting the trust relationships, and this could lead to serious and unexpected social misunderstanding.
%Especially, we should be cautious about recommending distrust because it can easily break some relationships that have been well maintained, i.e., ``\textit{trust is a fragile thing; it is easy to break, easy to lose and one of the hardest things to ever get back.}''
%%Our model effectively learns node embeddings considering multi-hop neighbor nodes under the signed random walks, and provides better predictive performance than other models; still more work is needed to  improve the prediction accuracy.

